Efficient Empowerment Estimation for Unsupervised Stabilization

Intrinsically motivated artificial agents learn advantageous behavior without externally-provided rewards. Previously, it was shown that maximizing mutual information between agent actuators and future states, known as the empowerment principle, enables unsupervised stabilization of dynamical systems at upright positions, which is a prototypical intrinsically motivated behavior for upright standing and walking. This follows from the coincidence between the objective of stabilization and the objective of empowerment. Unfortunately, sample-based estimation of this kind of mutual information is challenging. Recently, various variational lower bounds (VLBs) on empowerment have been proposed as solutions; however, they are often biased, unstable in training, and have high sample complexity. In this work, we propose an alternative solution based on a trainable representation of a dynamical system as a Gaussian channel, which allows us to efficiently calculate an unbiased estimator of empowerment by convex optimization. We demonstrate our solution for sample-based unsupervised stabilization on different dynamical control systems and show the advantages of our method by comparing it to the existing VLB approaches. Specifically, we show that our method has a lower sample complexity, is more stable in training, possesses the essential properties of the empowerment function, and allows estimation of empowerment from images. Consequently, our method opens a path to wider and easier adoption of empowerment for various applications.

==> Efficient Empowerment Estimation for Unsupervised Stabilization/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{Equation~\ref{#1}}  % Kevin changed this
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Efficient Empowerment Estimation for Unsupervised Stabilization/tex/Abstract.tex <==
\begin{abstract}
Intrinsically motivated artificial agents learn advantageous behavior without externally-provided rewards. Previously, it was shown that maximizing mutual information between agent actuators and future states, known as the empowerment principle, enables unsupervised stabilization of dynamical systems at upright positions, which is a prototypical intrinsically motivated behavior for upright standing and walking. This follows from the coincidence between the objective of stabilization and the objective of empowerment. Unfortunately, sample-based estimation of this kind of mutual information is challenging. Recently, various variational lower bounds (VLBs) on empowerment have been proposed as solutions; however, they are often biased, unstable in training, and have high sample complexity. In this work, we propose an alternative solution based on a trainable representation of a dynamical system as a Gaussian channel, which allows us to efficiently calculate an unbiased estimator of empowerment by convex optimization. We demonstrate our solution for sample-based unsupervised stabilization on different dynamical control systems and show the advantages of our method by comparing it to the existing VLB approaches. Specifically, we show that our method has a lower sample complexity, is more stable in training, possesses the essential properties of the empowerment function, and allows estimation of empowerment from images. Consequently, our method opens a path to wider and easier adoption of empowerment for various applications. \footnote{Project page: \url{https://sites.google.com/view/latent-gce}}

\end{abstract}

==> Efficient Empowerment Estimation for Unsupervised Stabilization/tex/Discussion.tex <==
\section{Summary and Discussion}\label{sec:Discussion}
In this work we introduce a new sample-based method for empowerment estimation in dynamical systems. The key component of our method is the representation of dynamical system by the Gaussian channel, which allows us to estimate empowerment by convex optimization. Our estimator converges to true empowerment landscape both from raw states and images. Empowerment is used in various applications and our improved estimator has a potential to improve these applications. For example in Appendix \ref{app:safety}, we show that when the agent is trained with an empowerment-aware objective, it develops distinguishable levels of attention to safety. Moreover, a natural continuation of this work is to learn skills using our representation of empowerment by Gaussian channel, rather than by VLB. 

==> Efficient Empowerment Estimation for Unsupervised Stabilization/tex/Experiments.tex <==
\section{Experiments}\label{sec:Experiments}
% In this section we compare different empowerment estimators, asking the following questions:
% \begin{itemize}
%     \item Does a particular estimator converge to ground truth empowerment?
%     \item What is the variance of a particular estimate in training? 
% \end{itemize}

\subsection{Unsupervised Stabilization of Classic Dynamic Systems}
As discussed in Section \ref{sec:intro}, a control policy that maximizes agent empowerment should lead to agent stabilization, even at an unstable equilibrium. To evaluate this, we compare our method with two prior works by \cite{mohamed2015variational} and \cite{Karl2019} on their ability to stabilize simple dynamic systems. Specifically, in the 2D ball-in-box environment, empowerment is highest at the center of the box, where the ball is free to move in all directions; in the pendulum environment, empowerment is highest at the up-right position, where gravity assists in reaching other states. We compare average squared distance away from the stable position during policy training. As shown in Figure \ref{fig:stabilization}, all three methods are successful on the simple ball-in-box environment, whereas only our method consistently stabilizes the pendulum at an unstable equilibrium. We refer readers to Appendix \ref{app:two_phase} for detailed visualization of pendulum empowerment/policy learning using our method, and Appendix \ref{app:cartpole_swing_up} for results on cart-pole.

\begin{figure}[h]
\centering
\includegraphics[trim=0px 0px 0px 20px, clip, width=0.35\textwidth]{images/bib-dist.png}
\includegraphics[trim=0px 0px 0px 20px, clip, width=0.35\textwidth]{images/pen-dist.png}
\vspace{-0.2cm}
\caption{Evaluating whether methods learn to stabilize simple dynamical systems. All methods succeed for ball-in-box, whereas only our method succeeds for pendulum.}
\label{fig:stabilization}
\end{figure}
\vspace{-0.2cm}

\subsection{Qualitative Convergence of Different Estimators}

We now qualitatively compare the convergence of different empowerment estimators to the true empowerment function. Not only do we include solutions by VLB methods that approximate the classic empowerment definition (\cite{mohamed2015variational, Karl2019}), but we also compare with recent works that employ empowerment-like objectives for skill discovery (\cite{eysenbach2018diversity, Sharma2020Dynamics-Aware}).
From Figure \ref{fig:emp_landscape}, we observe that in simple environments such as ball-in-box, all estimators converge to the correct landscape with high empowerment values in the middle and low values near the boundaries, corresponding to previous work (\cite{klyubin2005all}). For the pendulum environment, it is clear that while both the method by \cite{Karl2019} and ours succeed in creating results similar to the analytical solution (the ground truth), ours outputs an empowerment landscape that is smoother and more discerning. Detailed derivation of the analytical solution is included in Appendix \ref{app:G(s)}.

\begin{figure}[htb]
\centering
\includegraphics[width=1\linewidth]{images/emp_plots}
% \begin{subfigure}[t]{0.18\linewidth}
% \centering
% \includegraphics[trim=40px 20px 105px 20px, clip, height=2.2cm]{./images/bib-conv-ours.png}
% \end{subfigure}
% \begin{subfigure}[t]{0.18\linewidth}
% \centering
% \includegraphics[trim=40px 20px 105px 20px, clip, height=2.2cm]{./images/bib-conv-vim.png}
% \end{subfigure}
% \begin{subfigure}[t]{0.18\linewidth}
% \centering
% \includegraphics[trim=40px 20px 105px 20px, clip, height=2.2cm]{./images/bib-conv-Volkswagen.png}
% \end{subfigure}
% \begin{subfigure}[t]{0.18\linewidth}
% \centering
% \includegraphics[trim=40px 20px 105px 20px, clip, height=2.2cm]{./images/bib-conv-diayn.png}
% \end{subfigure}
% \begin{subfigure}[t]{0.18\linewidth}
% \centering
% \includegraphics[trim=40px 20px 60px 20px, clip, height=2.2cm]{./images/bib-conv-dads-q.png}
% \end{subfigure}

% \begin{subfigure}[t]{0.18\linewidth}
% \centering
% \includegraphics[trim=40px 20px 145px 20px, clip, height=2.2cm]{./images/pen-conv-ours.png}
% \caption{}
% \end{subfigure}
% \begin{subfigure}[t]{0.18\linewidth}
% \centering
% \includegraphics[trim=40px 20px 145px 20px, clip, height=2.2cm]{./images/pen-conv-vim.png}
% \caption{}
% \end{subfigure}
% \begin{subfigure}[t]{0.18\linewidth}
% \centering
% \includegraphics[trim=40px 20px 145px 20px, clip, height=2.2cm]{images/pen-conv-Volkswagen.png}
% \caption{}
% \end{subfigure}
% \begin{subfigure}[t]{0.18\linewidth}
% \centering
% \includegraphics[trim=40px 20px 105px 20px, clip, height=2.2cm]{images/pen-conv-diayn.png}
% \caption{}
% \end{subfigure}
% \begin{subfigure}[t]{0.18\linewidth}
% \centering
% \includegraphics[trim=40px 20px 60px 20px, clip, height=2.2cm]{images/pen-conv-dads-q.png}
% \caption{}
% \end{subfigure}
% \caption{Empowerment convergence by different methods (squashed linearly to [0, 1]). The top row plots the emp value of the 2D ball-in-box environment: x, y-axis correspond to the ball's position. The middle row is from the pendulum environment: x-axis: angle from to top in rad. y-axis: angular velocity in rad/s. (a) - ours, (b) - \cite{mohamed2015variational} (c) - \cite{Karl2019}, (d) - \cite{eysenbach2018diversity}, (e) - \cite{Sharma2020Dynamics-Aware}. \kl{include the ground truth here} \pz{TODO: replot + arrange images}}
\caption{Empowerment landscapes (normalized) for ball-in-box (top) and pendulum (bottom). In ball-in-box, central positions correspond to high empowerment. For pendulum, upright positions correspond to high empowerment; x-axis is the angle to top, y-axis is the angular velocity. From left to right, the plots show: ours, \cite{mohamed2015variational}, \cite{Karl2019}, \cite{eysenbach2018diversity}, \cite{Sharma2020Dynamics-Aware}.}
\vspace{-0.5cm}
\label{fig:emp_landscape}
\end{figure}

\subsection{Stability of Empowerment Estimations}
Besides the convergence to correct empowerment values, the stability and sample efficiency are also key aspects to determine whether the empowerment estimators are suitable as reliable intrinsic reward signals. We compute the variance of average empowerment values over 10 seeds as a measurement of algorithm stability. Since the outputs by existing methods are on different scales, we instead compare the relative standard deviation. As shown in Figure \ref{fig:variance}, our method outperforms the existing sample-based methods in that it has lower variance in training and faster convergence to the final estimator. These properties make our method competent as a reliable unsupervised training signal.

\begin{figure}[h!]
\centering
\includegraphics[width=.6\linewidth]{images/legend}
\\
\centering
\begin{subfigure}[t]{0.25\linewidth}
\centering
\includegraphics[trim=0px 0px 20px 20px, clip, height=2.7cm]{images/std-bib-log.png}
\caption{Ball-in-box}
\end{subfigure}
\begin{subfigure}[t]{0.23\linewidth}
\centering
\includegraphics[trim=30px 0px 20px 20px, clip, height=2.7cm]{images/std-pendulum-log.png}
\caption{Pendulum}
\end{subfigure}
\begin{subfigure}[t]{0.23\linewidth}
\centering
\includegraphics[trim=30px 0px 20px 20px, clip, height=2.7cm]{images/std-mountain-car-log.png}
\caption{Mountain car}
\end{subfigure}
\begin{subfigure}[t]{0.23\linewidth}
\centering
\includegraphics[trim=30px 0px 20px 20px, clip, height=2.7cm]{images/std-cartpole-log.png}
\caption{Cartpole}
\end{subfigure}
\caption{Relative standard deviation (RSD) in average empowerment value across 10 seeds. Our method converges faster to a lower RSD during training.}
\vspace{-0.5cm}
\label{fig:variance}
\end{figure}

\subsection{Empowerment Estimation in High-dimensional Systems}
We verify the applicability of Latent-GCE in high-dimensional systems from two aspects: first, the latent space should be invertible - able to predict the true underlying dynamics; moreover, the empowerment maximization policy should develop stabilizing behaviors.

\subsubsection{Pixel-based Pendulum}
We use a pendulum environment that supplies $64 \times 64$ images as observations. As input to our Latent-GCE algorithm, we concatenate two consecutive frames so as to capture the angular velocity. In Figure \ref{fig:reconstr}, we start the pendulum at its up-right position $s_0$. Using the encoder $f_{\chi}$, we map the images into the latent representation $f_{\chi}(s_0)$. Given different action sequences $a_0^H$, we predict the ending latent state as $z_{t+H} = G_{\chi}(f_{\chi}(s_t)) \cdot g_{\chi}(a_t^H)$. If our learned Latent-GCE model captures the true system dynamics, we expect the reconstruction of the ending state $f^{-1}_{\chi}(z_{t+H})$ to match the ground truth $s_{t+H}$.
This property holds true as verified in Figure \ref{fig:reconstr}. More importantly, as shown in Figure \ref{fig:pendulum_pixels}, the empowerment estimations given by our method is not only close to the analytical solution, but also trains a policy that swing the pendulum up from bottom to balance at the top. On the other hand, VIM by \cite{mohamed2015variational} which we compare as a baseline, fails to assign a high empowerment estimation for the up-right position.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\linewidth]{images/visualization.png}
    \caption{Reconstruction in the latent dynamics vs the ground truth. Starting from the same upright position, a different action sequence is taken in each row (action +1: counter-clockwise torque, 0: no torque, -1: clockwise torque). Reconstruction matches the actual observation in all cases.}
    \label{fig:reconstr}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[trim=0px 0px 110px 20px, clip, height=3cm]{images/pen-analytical-shifted.png}
    \includegraphics[trim=0px 0px 110px 20px, clip, height=3cm]{images/pen-pixel-ours.png}
    \includegraphics[trim=0px 0px 20px 20px, clip, height=3cm]{images/pen-pixel-vim.png}
    \caption{Empowerment estimates for pixel-based pendulum. Latent-GCE learns a reasonable empowerment function from pixels. Left: Analytical (x axis shifted by $\pi$ from Figure \ref{fig:emp_landscape}). Middle: Latent-GCE along with the swinging-up trajectory of the final control policy. Right: VIM.}
    \label{fig:pendulum_pixels}
\end{figure}

%In this section we demonstrate for the first time unsupervised stabilization by empowerment from images. Simply put, no prior work succeeded to estimate the empowerment function reliably from images for swinging up the pendulum and stabilizing it at the upright position, which has been demonstrated before only by the analytical empowerment calculation \cite{salge2013approximation}. Figure \ref{fig:pendfinal} shows the empowerment landscape computed from images by our approach, and the optimal trajectory for swinging up the pendulum from the bottom position to the upright position. The x-axis is $\theta$ (angle) and the y-axis is $\dot{\theta}$ (angular velocity). The black curve is the optimal trajectory for swinging up the pendulum, which starts from the bottom with $\theta=\SI{\pi}{\radian}$ and $\dot{\theta}=\SI{0}{\radian}$. At the beginning the pendulum swings with a small amplitude (the dense black dots around $\theta=\SI{\pi}{\radian}$, $\dot{\theta}=\SI{0}{\radian\per\second}$), then, once accumulated  enough energy, it starts traversing the state space, and arrives at the top position, where it stabilises, (dense black points around $\theta=\SI{0}{\radian}$, $\dot{\theta}=\SI{0}{\radian\per\second}$). 

\subsubsection{Hopper}
We evaluate the ability of Latent-GCE to stabilize the Hopper environment from OpenAI Gym. This environment is more challenging because of higher state dimension and long horizon (64) for empowerment estimation. Here we expect an empowerment maximization policy to balance the hopper at its standing position where it is able to move left and right freely. In Figure \ref{fig:hopper} we see our method successfully balances hopper whereas a random policy inevitably makes the hopper fall over.

\begin{figure}[h!]
    \centering
    \vspace{-0.3cm}
    \includegraphics[width=0.4\linewidth]{images/hopper-z-new.png}
    \caption{Average torso height over an evaluation episode of length 200 for the Hopper environment. Our method stabilizes the hopper to a standing position ($z \approx 1$).}
    \label{fig:hopper}
\end{figure}


==> Efficient Empowerment Estimation for Unsupervised Stabilization/tex/Introduction.tex <==
\section{Introduction}
\label{sec:intro}
Intrinsic motivation allows artificial and biological agents to acquire
useful behaviours without external knowledge (\cite{barto2004intrinsically, NIPS2004_2552, schmidhuber2010formal,  barto2013intrinsic,  oudeyer2016intrinsic}). In the framework of reinforcement learning (RL), this external knowledge is usually provided by an expert through a task-specific reward, which is optimized by an artificial agent towards a desired behavior (\cite{mnih2013dqn, 1707.06347}). 

In contrast, an intrinsic reward can arise solely from the interaction between the agent and environment, which eliminates the need for domain knowledge and reward engineering in some settings (\cite{mohamed2015variational, houthooft2017vime, pathak2017curiosity}). Previously, it was shown that maximizing mutual information (\cite{cover2012elements}) between an agent's actuators and sensors can guide the agent towards states in the environment with higher potential to achieve a larger number of eventual goals (\cite{klyubin2005all, wissner2013causal}). %This potential can be understood by the analogy to the question about a location of a fire station in a city, such that the firefighters will be able to respond to the largest number of eventual fires on average. \kl{For example, when choosing where to build a fire station, locations such that firefighters will be able to quickly respond to a large number of potential fires are preferable.}

Maximizing this kind of mutual information is known as the empowerment principle (\cite{1554676, salge2014empowerment}). Previously, it was found that an agent maximizing its empowerment converges to an unstable equilibrium of the environment in various dynamical control systems (\cite{jung2011empowerment,salge2013approximation,  Karl2019}). In this application, ascending the gradient of the empowerment function coincides with the objective of optimal control for stabilization at an unstable equilibrium (\cite{strogatz2018nonlinear}), which is an important task for both engineering (\cite{todorov2006optimal}) and biological\footnote{Broadly speaking, an increase in the rate of information flow in the perception-action loop (\cite{tishby2011information}) could be an impetus for the development of {\it homosapiens}, as hypothesized in (\cite{harari2014}).} systems; we refer to this as the \emph{essential property} of empowerment. It follows from the aforementioned prior works that a plausible estimate of the empowerment function should possess this essential property.

Empowerment has been found to be useful for a broad spectrum of applications, including: unsupervised skill discovery (\cite{Sharma2020Dynamics-Aware, eysenbach2018diversity, DBLP:conf/iclr/GregorRW17, Karl2019, EDL2020}; human-agent coordination (\cite{Salge2017EmpowermentAR,guckelsberger2016intrinsically});  assistance (\cite{AvE2020}); and stabilization (\cite{tiomkin2017control}).
% However, estimation of mutual information is hard (\cite{mcallester2018formal}). Fortunately, recent advances in deep learning (\cite{goodfellow2016deep}) have brought new opportunities for the estimation of mutual information from samples.
Past work has utilized variational lower bounds (VLBs) (\cite{poole2019variational, 45903, Tschannen2020On, mohamed2015variational}) to achieve an estimate of the empowerment. However, VLB approaches to empowerment in dynamical control systems (\cite{Sharma2020Dynamics-Aware, achiam2018valor}) have high sample complexity, are often unstable in training, and may be biased. Moreover, it was not previously studied if empowerment estimators learned via VLBs possess the essential properties of empowerment.

% In general, in these applications, the agent maximizes mutual information between its skills and one of: (1) its actuators, which generate either single actions (\cite{Karl2019,DBLP:conf/iclr/GregorRW17}) or (2) action sequences (\cite{tiomkin2017unified, salge2014empowerment}); (3) options (\cite{DBLP:conf/iclr/GregorRW17}); or (4) skills (\cite{Sharma2020Dynamics-Aware, eysenbach2018diversity}).
%There exist two possibilities for the estimation and use of empowerment: sequential and concurrent. In sequential mode, one first estimates empowerment before using it and/or its byproducts for downstream tasks (\cite{Sharma2020Dynamics-Aware, eysenbach2018diversity}). In concurrent mode, one estimates and uses empowerment simultaneously, which is adopted by our current work. The concurrent mode is suitable for scenarios when the empowerment objective coincides with the control objective, which happens for instance in stabilization. %%pa: can anything be said about our proposed approach also have potential in the other utilization scenario?

In this work, we introduce a new method, Latent Gaussian Channel Empowerment (Latent-GCE), for empowerment estimation and utilize the above-mentioned property as an ``indicator'' for the quality of the estimation. Specifically, we propose a particular representation for dynamical control systems using deep neural networks which is learned from state-action trajectories. This representation admits an efficient estimation of empowerment by convex optimization (\cite{cover2012elements}), both from raw state and from images. We propose an algorithm for simultaneous estimation and maximization of empowerment using standard RL algorithms such as Proximal Policy Optimization (\cite{1707.06347}), and Soft Actor-Critic (\cite{1801.01290}). We test our method on the task of unsupervised stabilization of dynamical systems with solely intrinsic reward, showing our estimator exhibits essential properties of the empowerment function.

% We believe our experiments clearly convey the gist of our method without losing the generality our estimator beyond the stabilization task; we discuss more general applications in the future directions.
We demonstrate the advantages of our method through comparisons to the existing state-of-the-art empowerment estimators in different dynamical systems from the OpenAI Gym simulator (\cite{1606.01540}). We find that our method (i) has a lower sample complexity, (ii) is more stable in training, (iii) possesses the essential properties of the empowerment function, and (iv) allows us to accurately estimate empowerment from images. We hope such a review of the existing methods for empowerment estimation will help push this research direction.

%The paper is organized as follows. In Section \ref{sec:Preliminaries} we review the necessary background on reinforcement learning, empowerment, and relevant existing works. In Section \ref{sec:Method} we explain our method. In Section \ref{sec:Experiments}, we provide numerical simulations of our method and comparison between our method to the existing state-of-the-art. In Section \ref{sec:Discussion} we summarize the paper, discuss the limitations of our method, and propose the continuation which is beyond the scope of the current work.  

==> Efficient Empowerment Estimation for Unsupervised Stabilization/tex/Method.tex <==
\section{Proposed Method}\label{sec:Method}
The desiderata for our method as follows:
\begin{itemize}
    \item to learn the channel matrix ($G(s)$ in \eqref{eq:GaussianChannel} from samples for arbitrary dynamics.
    \item to utilize general RL optimizers to reliably train intrinsically motivated policies.
    \item to enable empowerment maximization from arbitrary dynamics using latent representations.
\end{itemize}

These are desirable as: the ability to learn $G(s)$ from samples would allow us to estimate empowerment by the efficient line search algorithm in \eqref{eq:water_filling_solution}, recent advances in RL algorithms can alleviate challenges in stability and sample efficiency, and latent representations would allow our method to be applicable even when the observation or underlying dynamics do not satisfy the Gaussian Linear Channel assumption.

In this work, we present Latent Gaussian Channel Empowerment, or Latent-GCE in short. Schematically, our method is depicted in Figure \ref{fig:ours}. The controller policy $\pi_{\theta}(a\mid s)$ collects trajectories in the environment, $(s, a, s')$, where $s$ is either a state or image observation. The channel matrix $G_{\chi}(s_t)$ predicts the final state of a trajectory corresponding to the action sequence $a_t^{T-1}$, starting from $s_t$. After performing singular value decomposition on $G_{\chi}(s_t)$, the empowerment value $\mathcal{E}(s_t)$ is estimated by \eqref{eq:water_filling} and \eqref{eq:water_filling_solution}. The empowerment along trajectories provide intrinsic rewards, denoted by $r'(\tau)$, for the update of the controller policy, $\pi_{\theta}$, using off-the-shelf RL algorithms. Our method is summarized in high level in Algorithm \ref{alg:Latent-GCE}.
% \begin{wrapfigure}[15]{R}{0.6\textwidth}
\begin{figure}[t]
% \vspace{-0.55cm}
  \begin{center}
    \includegraphics[width=0.45\textwidth]{./images/ours.png}
  \end{center}
  \vspace{-0.3cm}
  \caption{Empowerment maximization via Latent-GCE}
  \label{fig:ours}
\end{figure}
% \end{wrapfigure}

\begin{algorithm}[h!]
\caption{Latent Gaussian Channel Empowerment Maximization}
\label{alg:Latent-GCE}
\begin{algorithmic}[1]
  \STATE {\bfseries Input:} $\pi_{\theta_0}(a\mid s)$ - control policy, $H$ - prediction horizon.
  \FOR{$i=0$ {\bfseries to} $N$}
  \STATE $\{\tau_k\}_{k=1}^K\leftarrow \mbox{run policy } \pi_{\theta_i}(a\mid s)$
  \hfill \COMMENT{data collection in environment}\\
  \STATE extract tuples $(s_t, \, a_t^{H-1}, \, s_{t+H})$ from $\{\tau_k\}_{k=1}^K$
  \hfill \COMMENT{data arrangement for Gaussian channel}\\
  \FOR{$j=1$ {\bfseries to} $M$}
  \STATE $\chi^* \leftarrow \underset{\chi}{\arg\min}\sum_{tuples}\left\Vert G_{\chi}(s_t) \cdot a_t^H - s_{t+H}\right\Vert^2_2$
  \hfill \COMMENT{projection to \eqref{eq:GaussianChannel}}\\
  \ENDFOR
  \STATE $\{\sigma_i^*(s_t)\}_{i=1}^k \leftarrow \mbox{SVD}(G_{\chi^*}(s_t))$
  \hfill \COMMENT{an alternative explained in Appendix \ref{app:svd_alternative}}\\
  \STATE $\mathcal{E}(s_t) \leftarrow \frac{1}{2}\sum_{i=1}^k \log(1 + \sigma^*_i(s)p^*_i)$
  \hfill \COMMENT{\eqref{eq:water_filling} and \eqref{eq:water_filling_solution}}\\
  \STATE reinforce $\pi_{\theta_i}(a\mid s)$ with $r'(\tau)=\sum_{t=1}^T\gamma^{t-1}\mathcal{E}(s_t)$.
  \hfill \COMMENT{policy update}\\
  \ENDFOR
\end{algorithmic}
\end{algorithm}

\subsection{Embedding of Observations and Action Sequences}
\label{sec:embbedding}
While the Gaussian Linear Channel defined in \eqref{eq:GaussianChannel} provides a good estimate of simple dynamic systems, we want our empowerment estimator to generalize to arbitrary dynamics, including high-dimensional systems, and environments where the observations are images. Using autoencoders, we embed the observations and action sequences such that their latent vector representations satisfy the Gaussian Linear Channel property. We use CNN encoder and decoder for image observations, or fully-connected networks for state observations. The encoder-decoder pair for action sequences are also parameterized by fully-connected networks. Let $f_{\chi}$, $f^{-1}_{\chi}$, $g_{\chi}$, $g^{-1}_{\chi}$ denote the encoder-decoder pairs for the observations and action sequences, $f_{\chi}$ maps the observations into $d_f$ dimensional latent states, and $g_{\chi}$ maps the $H$-step action sequences into $d_g$ dimensional latent actions. Our Latent Gaussian Linear Channel is formulated as follows:
\begin{align}
\label{eq:latent_gaussian_channel}
    f_{\chi}(s_{t+H}) = G_{\chi}(f_{\chi}(s_t)) \cdot g_{\chi}(a_t^H) + \eta
\end{align}

\subsection{Learning Channel Matrix G}
The channel matrix $G_{\chi}(f_{\chi}(s_t))$ has dimensions $d_f \times d_g$, where $d_f$ and $d_g$ are the dimensions of latent states and actions as defined in section \ref{sec:embbedding}. In the Latent Gaussian Linear Channel, as formulated in \eqref{eq:latent_gaussian_channel}, the ending latent state is approximated by a matrix-vector multiplication between the channel matrix $G_{\chi}(f_{\chi}(s_t))$ and the latent action $g_{\chi}(a_t^H)$. The mapping from a latent state to its channel matrix is parameterized by a 3-layer fully-connected neural network. The output layer of the network contains $d_f \cdot d_g$ neurons, which is then reshaped into the $d_f \times d_g$ matrix.

\subsection{Overall Optimization Objectives}
The overall training objective for our Latent-GCE estimation consists of two parts: reconstruction loss and latent prediction loss. The reconstruction loss $L_R$ is the average L2 distance between the decoded latent representations and the original encoder inputs. Minimizing $L_R$ encourages the autoencoders to learn meaningful latent representations. The prediction loss $L_P$ is the average L2 distance between the matrix-vector product and the true latent ending state. Minimizing $L_P$ forces the latent space to maintain the Gaussian Linear Channel structure:
\begin{align}
\label{eq:objective}
    L(\chi) = \hspace{0.1cm} &L_R + L_P \nonumber\\
    = \hspace{0.1cm} &\mathbb{E}_s\left\Vert f^{-1}_{\chi}(f_{\chi}(s)) - s\right\Vert^2_2 + \mathbb{E}_{a_t^H}\left\Vert g^{-1}_{\chi}(g_{\chi}(a_t^H)) - a_t^H\right\Vert^2_2 +\nonumber\\
    & \mathbb{E}_{(s_t, a_t^H, s_{t+H})}\left\Vert G_{\chi}(f_{\chi}(s_t)) \cdot g_{\chi}(a_t^H) - f_{\chi}(s_{t+H})\right\Vert^2_2
\end{align}

Overall, our Latent-GCE Maximization scheme (Figure \ref{fig:ours}) trains two sets of parameters, ($\theta$, $\chi$), while VLB methods (Figure \ref{fig:variational}) generally needs three sets, ($\theta$, $\phi$, $\psi$). The reduced trainable components suggest that our method might be superior in terms of better stability and quicker convergence, which we confirm in our experiment section.

% Comparing the empowerment estimation and maximization by VLB, depicted in Figure \ref{fig:variational}, and our method, depicted in Figure \ref{fig:ours}, the former is comprised of three neural networks, ($\theta$, $\phi$, $\psi$), while the latter involves only two networks, ($\theta$, $\chi$), plus, an efficient 1D line-search in \eqref{eq:water_filling_solution}. Strictly speaking, we propose a simpler scheme with less 'moving parts',  which is supposed to be more stable, as confirmed by the experiments in the next section.   



% \newpage

==> Efficient Empowerment Estimation for Unsupervised Stabilization/tex/Preamble.tex <==
\newtheorem{remark}{Remark}

\usepackage{wrapfig}


\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography

% Our Packages
\usepackage{graphicx}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{bbm}
\usepackage{caption}
\usepackage{subcaption}

% \usepackage[dvipsnames]{xcolor}

\usepackage{siunitx}

% \usepackage[skip=0pt]{caption}

\usepackage[export]{adjustbox}


\newcommand{\yy}[1]{{\color{BlueViolet}<YY: #1>}}
\newcommand{\pe}[1]{{\color{Cyan}<PE: #1>}}
\newcommand{\yd}[1]{{\color{Magenta}<YD: #1>}}
\newcommand{\pz}[1]{{\color{Red}<PZ: #1>}}
\newcommand{\kl}[1]{{\color{Green}<KL: #1>}}
\newcommand{\st}[1]{{\color{Blue}<ST: #1>}}

==> Efficient Empowerment Estimation for Unsupervised Stabilization/tex/Preliminaries.tex <==
\section{Preliminaries}\label{sec:Preliminaries}
In this section, we review the necessary background for our method, consisting of the reinforcement learning setting, various empowerment estimators, and the Gaussian channel capacity. We also review the underlying components in relevant prior work which we use for comparison to our method.  

% Also, we review the prior work, emphasizing the differences between them and our method.

\subsection{Reinforcement Learning}  %  and policy gradient algorithm}  % KL: there is no need to discuss policy gradient
\label{subsec:RL}

The reinforcement learning (RL) setting is modeled as an infinite-horizon Markov Decision Process (MDP) defined by: the state space $\mathcal{S}$, the action space $\mathcal{A}$, the transition probabilities $p(s' | s, a)$, the initial state distribution $p_0(s)$, the reward function $r(s, a) \in \mathbb{R}$, and the discount factor $\gamma$.
The goal of RL is to find an optimal control policy $\pi(a | s)$ that maximizes the expected return, i.e. $\max_{\pi} \; \mathbbm{E}_{s_0 \sim p_0, a_t \sim \pi, s_{t+1} \sim p} \bigl[\sum_{t=0}^{\infty} \gamma^t r(s_t, a_t) \bigr]$  (\cite{sutton2018reinforcement}). %In this work, we may assume instead that an intrinsic reward $r'$ is being optimized against, which may either be internal to the agent or provided; we will make this clear in the experiments.

% \begin{equation}
% \displaystyle \max_{\pi} \; \mathbbm{E}_{s_0 \sim p_0, a_t \sim \pi, s_{t+1} \sim p} \Bigl[\sum_{t=0}^{H-1} \gamma^t r(s_t, a_t) \Bigr],
% \end{equation}



\subsection{Empowerment}\label{subsec:Emp}
Interaction between an agent and its environment is plausibly described by the perception-action cycle (PAC), (\cite{tishby2011information}), where the agent observes the state of the environment via its sensors and responds with its actuators. The maximal information rate from actuators to sensors is an inherent property of PAC which characterizes the \textit{empowerment} of the agent, formally defined below.     

Empowerment (\cite{klyubin2005all}) is defined by the maximal mutual information rate (\cite{cover2012elements}) between the agent's sensor observations $o\in \mathcal{O}$ and actuators $a\in \mathcal{A}$ given the current state $s\in \mathcal{S}$. It is fully specified by a fixed probability distribution of sensor observations conditioned on the actuators and the state, $p(O \mid A, s)$, denoted by ``channel'',  and by a free probability of the actuator signals conditioned on the state, $\omega(A \mid s)$, denoted by ``source''. The empowerment $\mathcal{E}$ is the capacity of the channel, which is found via optimization of the source distribution $\omega(A \mid s)$:
\begin{align}\label{eq:emp_definition}
   \mathcal{E}(s) = \underset{\omega(A \mid s)}{\max} \;\mathcal{I}[O; A \mid s]=\underset{\omega(A \mid s)}{\max}\sum_{O, A}p(O, A\mid s)\log\Biggl(\frac{p(A\mid O, s)}{\omega(A\mid s)}\Biggr)
\end{align}
where $\mathcal{I}[O; A \mid s]$ is the mutual information, reflecting the difference between the entropy of the sensor inputs, $\mathcal{H}(O\mid s)$ and the corresponding conditional entropy,  $\mathcal{H}(O\mid A, s)$\footnote{when the agent does not have an access to the true state, $s$, empowerment is calculated as the maximal mutual information between actuators and sensors given an estimated state.}.
% \kl{are $s$ and $o$ drawn from the same distribution (ex. both images?) if so, could this be made more clear/if not, do you have to estimate state? in typical RL notation $O$ refers to a partial observation of $s$}
% \st{When the agent does not have an access to the true state, $s$, then empowerment is calculated as the maximal mutual information between actuators and sensors given an estimated state.}

In this work, we follow the original empowerment formulation (\cite{klyubin2005all}), where $A$ is an action sequence of length $T$ starting from the state $s$ and $O$ is the resulting observation sequence. However, our method is applicable to other choices of observation and control sequences. 

\begin{remark}\label{rem:3_policies}
The source distribution in \eqref{eq:emp_definition}, $\omega^*(A \mid s)$, is used only for the estimation of empowerment. Another policy, $\pi(a\mid s)$, is calculated using empowerment as an intrinsic reward by either reinforcement learning (\cite{Karl2019}) or a 1-step greedy algorithm (\cite{jung2011empowerment, salge2013approximation}) to reach the states with maximal empowerment. Strictly speaking, the source distribution $\omega$ maximizes the mutual information, (i.e. estimates the empowerment), while the policy distribution $\pi$ maximizes expected accumulated empowerment along trajectories.      
\end{remark}

In general, the capacity of an arbitrary channel for a continuous random variable is unknown except for a few special cases such as the Gaussian linear channel, as reviewed below. As a result, past works have largely relied on variational lower bounds instead.

\subsubsection{Empowerment by Variational Lower Bounds}\label{subsubsec:VLB}
The mutual information in \eqref{eq:emp_definition} can be bounded from below as follows (\cite{mohamed2015variational,  DBLP:conf/iclr/GregorRW17, Karl2019, poole2019variational}):

{\small
\begin{align}\label{eq:VLB1}
\sum_{O, A}p(O, A\mid s)\log\Bigl(\frac{p(A\mid O, s)}{\omega(A\mid s)}\Bigr) &= \sum_{O, A}p(O, A\mid s)\log\Bigl(\frac{q(A\mid O, s)}{\omega(A\mid s)}\Bigr) 
+ D_{KL}\left[p(A\mid O, s) \mid\mid q(A\mid O, s)\right]\nonumber\\
&\le \sum_{O, A}p(O, A\mid s)\log\Bigl(\frac{q(A\mid O, s)}{\omega(A\mid s)}\Bigr)
\end{align}
}

where $q(A\mid O, s)$ and $\omega(A\mid s)$ are represented by neural networks with parameters $\phi$ and $\psi$ respectively. The lower bound in \eqref{eq:VLB1} can be estimated from samples using reinforcement learning with intrinsic reward $r(s_t, a_t) = \sum_t^T \log q_{\phi}(a_t\mid o_t, s) - \log \omega_{\psi}(a_t\mid s_t)$, as detailed in (\cite{DBLP:conf/iclr/GregorRW17, Karl2019}). To apply this variational lower bound on empowerment to unsupervised stabilization of dynamical systems one needs to learn three distributions: $q_{\phi}(a_t\mid o_t, s)$ and $\omega_{\psi}(a_t\mid s_t)$ for the lower bound in \eqref{eq:VLB1}, and $\pi(a\mid s)$ as the control policy (see Remark \ref{rem:3_policies}).

Developing the mutual information in \eqref{eq:emp_definition} in the opposite direction, one gets another lower bound on empowerment, an approximation of which was used in (\cite{Sharma2020Dynamics-Aware}):

{\small
\begin{align}\label{eq:VLB2} 
\sum_{O, A}p(O, A\mid s)\log\Bigl(\frac{p(O\mid A, s)}{\omega(O\mid s)}\Bigr) &= \sum_{O, A}p(O, A\mid s)\log\Bigl(\frac{q(O\mid A, s)}{\omega(O\mid s)}\Bigr)\nonumber 
+ D_{KL}\left[p(O\mid A, s) \mid\mid q(O\mid A, s)\right]\nonumber\\
&\le \sum_{O, A}p(O, A\mid s)\log\Bigl(\frac{q(O\mid A, s)}{\omega(O\mid s)}\Bigr).
\end{align}
}

\begin{figure}[t]
    \begin{center}
        \includegraphics[width=0.45\textwidth]{./images/variational.png}
    \end{center}
    \vspace{-0.3cm}
    \caption{Estimation of empowerment via variational lower bounds.}
    \label{fig:variational}
    \vspace{-0.3cm}
\end{figure}

% \begin{wrapfigure}[14]{R}{0.6\textwidth}
% \vspace{-0.15cm}
% \end{wrapfigure}

For sake of the clarity of the exposition, the above-explained variational empowerment is schematically depicted in Figure \ref{fig:variational}. The controller policy, $\pi_{\theta}(a\mid s)$, collects transitions in environment, $(s, a, s')$. The source policy $\omega_{\psi}(a\mid s)$ generates the action $a$ at every state $s$ visited by the controller policy, and the environment transits to the next state, $s'$ (yellow block). The inverse channel policy $q_{\phi}(a\mid s, s')$ is regressed to $a$ given $s$ and and $s'$, generating the intrinsic reward, $C=\log \omega_{\psi}(a\mid s) - \log q_{\phi}(a\mid s, s')$, which is used as the reward to improve the controller policy via reinforcement learning. This scheme aims to transfer the intrinsically motivated agent to the state of the maximal empowerment in the environment. 

\subsubsection{Empowerment for Gaussian Channels}\label{subsubsec:Capacity}
The Gaussian linear channel in our case is given by:
\begin{align}\label{eq:GaussianChannel}
    O = G(s)\cdot A + \eta,
\end{align}
where $O$ and $A$ are the observation and actuator sequences with dimensions $d_O\times 1$ and $d_A\times 1$, respectively; $G(s)$ is a matrix with dimensions $d_O\times d_A$; and $\eta$ is multivariate Gaussian noise with dimension $d_O\times 1$. Following \cite{salge2013approximation}, we assume the noise is distributed as a Gaussian. For completeness, Appendix \ref{app:G(s)} provides the analytical derivation of $G(s)$ in the case of known dynamics for pendulum for the action sequence $A$ with length 3. In contrast, the current work proposes a method how to estimate $G(s)$ for arbitrary dynamics and arbitrary length of the action sequence from samples. The details of the calculation of Gaussian channel capacity are included in Appendix \ref{app:GaussianChannel}.

The key observation in our method is that we can learn $G(s)$ from samples, which allows us to estimate empowerment efficiently for arbitrary dynamics, including for high-dimensional dynamical systems or from images (pixels). As a result, it is not required to resort to lower bounds as done in prior work. In Section \ref{sec:Method}, we describe how to learn $G(s)$ from samples using deep neural networks. % The appropriateness of \eqref{eq:GaussianChannel} for empowerment estimation has been studied in \cite{salge2013approximation}, where the dynamics was known and the state was fully observable. These assumptions allow analytical computation of empowerment for certain dynamical systems, which provides us with the ground truth empowerment landscapes in Section \ref{sec:Experiments}.    


==> Efficient Empowerment Estimation for Unsupervised Stabilization/tex/PriorWorks.tex <==
\section{Related Work}\label{subsec:Prior Work}
% \vspace{-0.3cm}
In this section, we review the relevant prior work and state of the art in empowerment estimation, emphasizing the main differences between these existing works and our proposed approach.

\paragraph{Estimation via Gaussian channel.}
The representation given by \eqref{eq:GaussianChannel} was previously considered in (\cite{salge2013approximation}), where the channel $p(O \mid A, s)$ was assumed to be known. In our current work, we remove this assumption and extend the applicability of the efficient channel capacity solution given by \eqref{eq:water_filling} to arbitrary observations, including images.

\paragraph{Variational approaches to estimation.}
The lower bound in \eqref{eq:VLB1} is used in (\cite{mohamed2015variational, DBLP:conf/iclr/GregorRW17, Karl2019}), where different additional assumptions are made. Specifically, \cite{mohamed2015variational} estimates empowerment in open loop, while \cite{DBLP:conf/iclr/GregorRW17, Karl2019} provide a solution for closed-loop empowerment, and \cite{Karl2019} assumes differentiability of the dynamics. In our work, we do not assume differentiable dynamics and we do not resort to variational bounds, aiming to achieve a more stable, sample-efficient, and generalizable estimator of empowerment without losing the essential properties of the empowerment function, as explained in the Introduction. The works by (\cite{mohamed2015variational,DBLP:conf/iclr/GregorRW17}) precede that by (\cite{Karl2019}), and we also experimentally find the latter to be more stable. Consequently, in Section \ref{sec:Experiments} we provide comparisons to \cite{Karl2019}, which represents the current start of the art in this line of research.
 
\paragraph{Skill discovery.}
An approximation of the lower bound in \eqref{eq:VLB2} is successfully used by \cite{Sharma2020Dynamics-Aware} in the context of learning a set of skills. Another relevant and important work is \cite{eysenbach2018diversity}. Citing the authors, their work is about \textit{``maximizing the empowerment of a hierarchical agent whose action space is the set of skills''}. Section \ref{sec:Experiments} provides comparisons between our empowerment estimator and these methods with regards to stability in training, sample efficiency, and correctness of the empowerment landscape generated by both methods. Although they aim to achieve a different goal from our work -- unsupervised skill discovery vs unsupervised stabilization -- their objectives are the same type us ours: maximizing mutual information between actuators and sensors. In Section \ref{sec:Experiments} we show that the empowerment landscape derived by these methods converge to the true empowerment landscape in simple cases, but fail to converge to a known empowerment landscape in more complicated dynamical systems.
 
% Specifically, they suggest maximizing a variational lower bound in the form of \eqref{eq:VLB1} on the mutual information between skills and states with an additional term of conditional entropy of actions given skills and states, $\mathcal{H}(A|S, Z)$, (which is equal to zero for a deterministic policy).    

% A recent work by \citet{qureshi2018adversarial} applies empowerment to Inverse Reinforcement Learning. Their results show that when empowerment is used along with reward and policy learning, IRL manages to learn near-optimal control policies and robust reward functions, which are superior to those from the existing methods. Our improved empowerment estimation can be useful in this hybrid, (intrinsic and extrinsic) setting, which we deter to the future work. \kl{does this belong here? can we discuss applications in the discussion later?}
 
These works represent the state of the art in empowerment estimation. We believe a thorough comparison between our method and these works, as provided in Section \ref{sec:Experiments}, clearly demonstrate the main properties of our method and clarify our contribution to the improvement of sample-based empowerment estimation in dynamical systems. As mentioned in the introduction, empowerment is useful for a broad spectrum of different applications. In this section, we highlighted the most relevant and updated methods, which we hope are helpful to see the merits and advances of our approach.

% \kl{another work that may be of interest is \cite{berseth2020smirl}, which learns with intrinsic reward to minimize entropy for environments where good performance comes from stability: they show Tetris, staying alive in a shooting game, not falling off a clisp; from pixels}

Our improved empowerment estimation possesses the essential properties of the empowerment function: in particular, it converges to the correct empowerment landscape. The training has improved stability. Furthermore, it allows for the estimation of the empowerment function from images, which we demonstrate in Section \ref{sec:Experiments}, where we show purely intrinsically motivated (empowerment-based) stabilization of inverted pendulum from images. Accurate estimation of empowerment from images significantly expands the possible breadth of applications for empowerment. % In the next section, we explain our method, referring to the background reviewed in this section.

==> Efficient Empowerment Estimation for Unsupervised Stabilization/tex/bck/Introduction.tex.bck.01 <==
\section{Introduction}
Intrinsic motivation allows artificial and biological agents to acquire
useful behaviours without external  knowledge (\cite{schmidhuber2010formal, barto2004intrinsically, barto2013intrinsic, NIPS2004_2552, oudeyer2016intrinsic}). In the framework of reinforcement learning, (RL), this external domain knowledge is usually provided by an expert through task specific reward, which is optimised by an artificial agent towards desired behaviour. This form of RL is successfully applied to different scenarios [Philip, Kevin, put please here a few generic updated citations \cite{mnih2013dqn, 1707.06347})] \kl{is this sentence necessary?}\st{NO. in general, we should keep only the necessary sentences, all what can be removed should go out! We can move the citations on RL to the previous sentence.}. The main disadvantages of this approach are the need to obtain domain knowledge for new environments, and poor generalization to other tasks \kl{I am not sure this is relevant to the benefits of this work} \footnote{The latter can alleviated by meta-learning (\cite{finn2017model}), and goal-conditional policies (\cite{nasiriany2019planning}), which is orthogonal to the main focus of the current work***}.  

In contrast, intrinsic reward can arise solely from the interaction between the agent and environment [REFS] (\cite{mohamed2015variational, houthooft2017vime, pathak2017curiosity}). Previously, it was shown that maximizing mutual information between agent actuators and its sensors reveals preferable states in environment with regard to the potential to achieve from them a larger number of eventual goals (\cite{wissner2013causal, klyubin2005all}). This potential can be understood by the analogy to the question about where to locate a fire station in a city, such that the firefighters will be able to respond to the largest number of eventual fires on average. Information theoretical quantities allow us to operate with abstract spaces, (such as graph, manifold, language, skill, action, option) through probability distribution, which generalizes the question about positions in Euclidean spaces to points in probability simplex (\cite{cover2012elements}). The subject of this work is intrinsic reward which reflects this potential, and is quantified by the mutual information between actuators and sensors.  

Maximizing this kind of mutual information is known as the empowerment principle (\cite{1554676, salge2014empowerment}). Empowerment is a function of state. It was shown in (\cite{salge2013approximation, jung2011empowerment, Karl2019}) that an agent maximizing its empowerment converges to unstable equilibrium of environment. That was demonstrated on pendulum, pole on a cart, acrobot, balls in a box, bicycle, bipedal walker and other \kl{simplify to ``various'' instead of listing?} dynamical control systems (\cite{salge2013approximation, jung2011empowerment, Karl2019}). In this sense, ascending the gradient of the empowerment function towards unstable equilibrium coincides with the objective of optimal control for stabilization at unstable equilibrium (\cite{strogatz2018nonlinear}) \kl{was it going to be mentioned somewhere around here that empowerment objective is automatically generated for environments, rather than having to hand engineer expert reward functions?}, which is an important task for both engineering (\cite{todorov2006optimal}) and biological\footnote{Broadly speaking, an increase in the rate of information flow in the perception-action loop (\cite{tishby2011information}) could be an impetus for the development of {\it homosapiens}, as hypothesized in (\cite{harari2014}).} systems. It follows from the above mentioned prior works on empowerment that a plausible estimate of the empowerment function should possess this essential property of empowerment. \kl{maybe the last two paragraphs can be made more brief and combined; both describe the empowerment principle (fire station analogy is quite long, and also described as unstable equilibriums)}

    

Empowerment was found useful for a broad spectrum of applications. Among others are unsupervised skill discovery (\cite{Sharma2020Dynamics-Aware, eysenbach2018diversity, DBLP:conf/iclr/GregorRW17, Karl2019, EDL2020}), human-agent coordination (\cite{Salge2017EmpowermentAR,guckelsberger2016intrinsically}),  assistance (\cite{AvE2020}), and stabilization (\cite{tiomkin2017control}). In general, in these applications, an agent maximizes mutual information between its actuators, (generating either action sequence as in (\cite{tiomkin2017unified, salge2014empowerment}), or options as in (\cite{DBLP:conf/iclr/GregorRW17}), or skills as in (\cite{Sharma2020Dynamics-Aware, eysenbach2018diversity})) and its sensors. The same objective, (the empowerment function), is optimized by the agent in the above-mentioned applications, while the difference between these them is in optimization machinery, conditional dependency between random variables, and the structure of control signal, which comprises either action sequences, or options, or skills \kl{is this sentence unique from the last one?} \st{i see. will merge these two sentences} .

In addition, there are two possibilities for estimation and utilization of empowerment: sequential and concurrent. In sequential mode, one firstly estimates empowerment, then utilizes it and/or its byproducts for downstream tasks (\cite{Sharma2020Dynamics-Aware, eysenbach2018diversity}). In concurrent mode, one estimates and utilizes empowerment simultaneously, which is adopted by the current work as well. The concurrent mode is more suitable when the the empowerment objective coincides with the control objective, which happens for instance in stabilization.      

Estimation of mutual information is hard (\cite{mcallester2018formal}). Fortunately, recent advances in deep neural networks (\cite{goodfellow2016deep}) have brought new opportunities for the estimation of mutual information from samples by means of variational low bounds, (VLB), (\cite{poole2019variational, 45903, Tschannen2020On, mohamed2015variational}). However, VLB on empowerment in dynamical control systems (\cite{Sharma2020Dynamics-Aware, achiam2018valor}, [REFS]) have high sample complexity, are often unstable in training \kl{the DADS-Off off policy version of DADS improves on these first two aspects significantly}, and may have a bias [refs] \kl{not sure why there are citations here, VLB is biased by nature?}. Moreover, it was not confirmed previously that VLBs on empowerment do preserve the essential properties of the empowerment function. 

In this work we introduce a new method for empowerment estimation from samples, and utilise the above mentioned property as an "indicator" for the quality of empowerment estimation. Specifically, we propose an alternative path to the estimation of empowerment in dynamical control system, which is based on a particular representation of dynamical control systems by deep neural networks, rather than on VLB. This representation is learnt from samples, (states and actions), and it admits an efficient estimation of empowerment by convex optimization (\cite{cover2012elements}). We propose a unified, (the above mentioned concurrent mode), approach for simultaneous estimation and maximization of empowerment by the off-the-shelf optimisers such as Policy Proximity Optimization, (\cite{1707.06347}) and Stochastic Actor Critic (\cite{1801.01290}). Our method allows us to construct this representation of dynamical systems both from raw states and from images, as demonstrated by numerical simulations.  

Our method is a generic sample-based empowerment estimator. For the sake of clearance of the exposition, and due to the above-mentioned plethora of the possibilities and the applications of empowerment, we put our method on a dedicated testbed, addressing the essential property of the empowerment function, which is the ability to solve the stabilization task with intrinsic reward only.

We believe our experiments convey to the readers in the best way the gist of our method without losing the generality of applicability of our estimator beyond the stabilization task, as we discuss in the future directions.
We demonstrate the advantages of our method by thorough comparisons to the existing state-of-the-art empowerment estimators in different dynamical systems. We found that i) our method has a lower sample complexity, ii) it is more stable in training, iii) it does possess the essential properties of the empowerment function, (while the existing methods do not necessarily do, even though their objective is empowerment maximization as well).

The paper is organised as follows. In Section \ref{sec:Preliminaries} we review the necessary background on reinforcement learning, empowerment, and relevant existing works. In Section \ref{sec:Method} we explain our method. In Section \ref{sec:Experiments}, we provide a) numerical simulations of our method, and) comparison between our method and the existing methods. In Section \ref{sec:Discussion} we summarize the paper, discus the limitations of our method, and propose the continuation which is beyond the scope of the current work.  


==> Efficient Empowerment Estimation for Unsupervised Stabilization/tex/bck/Introduction.tex.bck.02 <==
\section{Introduction}
Intrinsic motivation allows artificial and biological agents to acquire
useful behaviours without external knowledge (\cite{barto2004intrinsically, NIPS2004_2552, schmidhuber2010formal,  barto2013intrinsic,  oudeyer2016intrinsic}). In the framework of reinforcement learning, (RL), this external domain knowledge is usually provided by an expert through task specific reward, which is optimised by an artificial agent towards desired behaviour (\cite{mnih2013dqn, 1707.06347}). 
% The main disadvantages of this approach are the need to obtain domain knowledge for new environments, and poor generalization to other tasks \kl{I am not sure this is relevant to the benefits of this work} \footnote{The latter can alleviated by meta-learning (\cite{finn2017model}), and goal-conditional policies (\cite{nasiriany2019planning}), which is orthogonal to the main focus of the current **}.  

In contrast, intrinsic reward can arise solely from the interaction between the agent and environment, which eliminate in certain scenarios the need in domain knowledge and reward engineering (\cite{mohamed2015variational, houthooft2017vime, pathak2017curiosity}). Previously, it was shown that maximizing mutual information between agent actuators and its sensors reveals preferable states in environment with regard to the potential to achieve from them a larger number of eventual goals (\cite{klyubin2005all, wissner2013causal}). This potential can be understood by the analogy to the question about where to locate a fire station in a city, such that the firefighters will be able to respond to the largest number of eventual fires on average. Information theoretical quantities allow us to operate with abstract spaces, (such as graph, manifold, language, skill, action, option) through probability distribution, which generalizes the question about positions in Euclidean spaces to points in probability simplex (\cite{cover2012elements}). The subject of this work is intrinsic reward which reflects this potential, and is quantified by the mutual information between actuators and sensors.  

Maximizing this kind of mutual information is known as the empowerment principle (\cite{1554676, salge2014empowerment}). Empowerment is a function of state. It depends only on the properties of agent and environment. Previously, it was shown that an agent maximizing its empowerment converges to unstable equilibrium of environment which was demonstrated on various dynamical control systems (\cite{jung2011empowerment,salge2013approximation,  Karl2019}). In this sense, ascending the gradient of the empowerment function towards unstable equilibrium coincides with the objective of optimal control for stabilization at unstable equilibrium (\cite{strogatz2018nonlinear}) \kl{was it going to be mentioned somewhere around here that empowerment objective is automatically generated for environments, rather than having to hand engineer expert reward functions?}, which is an important task for both engineering (\cite{todorov2006optimal}) and biological\footnote{Broadly speaking, an increase in the rate of information flow in the perception-action loop (\cite{tishby2011information}) could be an impetus for the development of {\it homosapiens}, as hypothesized in (\cite{harari2014}).} systems. It follows from the above mentioned prior works on empowerment that a plausible estimate of the empowerment function should possess this essential property of empowerment. \kl{maybe the last two paragraphs can be made more brief and combined; both describe the empowerment principle (fire station analogy is quite long, and also described as unstable equilibrium)}

    

Empowerment was found useful for a broad spectrum of applications. Among others are unsupervised skill discovery (\cite{Sharma2020Dynamics-Aware, eysenbach2018diversity, DBLP:conf/iclr/GregorRW17, Karl2019, EDL2020}), human-agent coordination (\cite{Salge2017EmpowermentAR,guckelsberger2016intrinsically}),  assistance (\cite{AvE2020}), and stabilization (\cite{tiomkin2017control}). In general, in these applications, the agent maximizes mutual information between its actuators, which generate either action as in (\cite{Karl2019,DBLP:conf/iclr/GregorRW17}), or action sequence as in (\cite{tiomkin2017unified, salge2014empowerment}), or options as in (\cite{DBLP:conf/iclr/GregorRW17}), or skills as in (\cite{Sharma2020Dynamics-Aware, eysenbach2018diversity}) and its sensors. 

In addition, there are two possibilities for estimation and utilization of empowerment: sequential and concurrent. In sequential mode, one firstly estimates empowerment, then utilizes it and/or its byproducts for downstream tasks (\cite{Sharma2020Dynamics-Aware, eysenbach2018diversity}). In concurrent mode, one estimates and utilizes empowerment simultaneously, which is adopted by the current work as well. The concurrent mode is more suitable when the the empowerment objective coincides with the control objective, which happens for instance in stabilization.      

Estimation of mutual information is hard (\cite{mcallester2018formal}). Fortunately, recent advances in deep neural networks (\cite{goodfellow2016deep}) have brought new opportunities for the estimation of mutual information from samples by means of variational low bounds, (VLB), (\cite{poole2019variational, 45903, Tschannen2020On, mohamed2015variational}). However, VLB on empowerment in dynamical control systems (\cite{Sharma2020Dynamics-Aware, achiam2018valor}) have high sample complexity, are often unstable in training, and may have a bias. Moreover, it was not confirmed previously that VLBs on empowerment do preserve the essential properties of the empowerment function. 

In this work we introduce a new method for empowerment estimation from samples, and utilise the above mentioned property as an "indicator" for the quality of empowerment estimation. Specifically, we propose an alternative path to the estimation of empowerment in dynamical control system, which is based on a particular representation of dynamical control systems by deep neural networks, rather than on VLB. This representation is learnt from samples, (states and actions), and it admits an efficient estimation of empowerment by convex optimization (\cite{cover2012elements}). We propose a unified, (the above mentioned concurrent mode), approach for simultaneous estimation and maximization of empowerment by the off-the-shelf optimisers such as Policy Proximity Optimization, (\cite{1707.06347}) and Stochastic Actor Critic (\cite{1801.01290}). Our method allows us to construct this representation of dynamical systems both from raw states and from images, as demonstrated by numerical simulations.  

Our method is a generic sample-based empowerment estimator. For the sake of clearance of the exposition, and due to the above-mentioned plethora of the possibilities and the applications of empowerment, we put our method on a dedicated testbed, addressing the essential property of the empowerment function, which is the ability to solve the stabilization task with intrinsic reward only.

We believe our experiments convey to the readers in the best way the gist of our method without losing the generality of applicability of our estimator beyond the stabilization task, as we discuss in the future directions. We demonstrate the advantages of our method by thorough comparisons to the existing state-of-the-art empowerment estimators in different dynamical systems. We found that i) our method has a lower sample complexity, ii) it is more stable in training, iii) it does possess the essential properties of the empowerment function, while the existing methods do not.

The paper is organised as follows. In Section \ref{sec:Preliminaries} we review the necessary background on reinforcement learning, empowerment, and relevant existing works. In Section \ref{sec:Method} we explain our method. In Section \ref{sec:Experiments}, we provide a) numerical simulations of our method, and) comparison between our method and the existing methods. In Section \ref{sec:Discussion} we summarize the paper, discus the limitations of our method, and propose the continuation which is beyond the scope of the current work.  

==> tex/bck/Introduction.tex.bck.01 <==
\section{Introduction}
Intrinsic motivation allows artificial and biological agents to acquire
useful behaviours without external  knowledge (\cite{schmidhuber2010formal, barto2004intrinsically, barto2013intrinsic, NIPS2004_2552, oudeyer2016intrinsic}). In the framework of reinforcement learning, (RL), this external domain knowledge is usually provided by an expert through task specific reward, which is optimised by an artificial agent towards desired behaviour. This form of RL is successfully applied to different scenarios [Philip, Kevin, put please here a few generic updated citations \cite{mnih2013dqn, 1707.06347})] \kl{is this sentence necessary?}\st{NO. in general, we should keep only the necessary sentences, all what can be removed should go out! We can move the citations on RL to the previous sentence.}. The main disadvantages of this approach are the need to obtain domain knowledge for new environments, and poor generalization to other tasks \kl{I am not sure this is relevant to the benefits of this work} \footnote{The latter can alleviated by meta-learning (\cite{finn2017model}), and goal-conditional policies (\cite{nasiriany2019planning}), which is orthogonal to the main focus of the current work***}.  

In contrast, intrinsic reward can arise solely from the interaction between the agent and environment [REFS] (\cite{mohamed2015variational, houthooft2017vime, pathak2017curiosity}). Previously, it was shown that maximizing mutual information between agent actuators and its sensors reveals preferable states in environment with regard to the potential to achieve from them a larger number of eventual goals (\cite{wissner2013causal, klyubin2005all}). This potential can be understood by the analogy to the question about where to locate a fire station in a city, such that the firefighters will be able to respond to the largest number of eventual fires on average. Information theoretical quantities allow us to operate with abstract spaces, (such as graph, manifold, language, skill, action, option) through probability distribution, which generalizes the question about positions in Euclidean spaces to points in probability simplex (\cite{cover2012elements}). The subject of this work is intrinsic reward which reflects this potential, and is quantified by the mutual information between actuators and sensors.  

Maximizing this kind of mutual information is known as the empowerment principle (\cite{1554676, salge2014empowerment}). Empowerment is a function of state. It was shown in (\cite{salge2013approximation, jung2011empowerment, Karl2019}) that an agent maximizing its empowerment converges to unstable equilibrium of environment. That was demonstrated on pendulum, pole on a cart, acrobot, balls in a box, bicycle, bipedal walker and other \kl{simplify to ``various'' instead of listing?} dynamical control systems (\cite{salge2013approximation, jung2011empowerment, Karl2019}). In this sense, ascending the gradient of the empowerment function towards unstable equilibrium coincides with the objective of optimal control for stabilization at unstable equilibrium (\cite{strogatz2018nonlinear}) \kl{was it going to be mentioned somewhere around here that empowerment objective is automatically generated for environments, rather than having to hand engineer expert reward functions?}, which is an important task for both engineering (\cite{todorov2006optimal}) and biological\footnote{Broadly speaking, an increase in the rate of information flow in the perception-action loop (\cite{tishby2011information}) could be an impetus for the development of {\it homosapiens}, as hypothesized in (\cite{harari2014}).} systems. It follows from the above mentioned prior works on empowerment that a plausible estimate of the empowerment function should possess this essential property of empowerment. \kl{maybe the last two paragraphs can be made more brief and combined; both describe the empowerment principle (fire station analogy is quite long, and also described as unstable equilibriums)}

    

Empowerment was found useful for a broad spectrum of applications. Among others are unsupervised skill discovery (\cite{Sharma2020Dynamics-Aware, eysenbach2018diversity, DBLP:conf/iclr/GregorRW17, Karl2019, EDL2020}), human-agent coordination (\cite{Salge2017EmpowermentAR,guckelsberger2016intrinsically}),  assistance (\cite{AvE2020}), and stabilization (\cite{tiomkin2017control}). In general, in these applications, an agent maximizes mutual information between its actuators, (generating either action sequence as in (\cite{tiomkin2017unified, salge2014empowerment}), or options as in (\cite{DBLP:conf/iclr/GregorRW17}), or skills as in (\cite{Sharma2020Dynamics-Aware, eysenbach2018diversity})) and its sensors. The same objective, (the empowerment function), is optimized by the agent in the above-mentioned applications, while the difference between these them is in optimization machinery, conditional dependency between random variables, and the structure of control signal, which comprises either action sequences, or options, or skills \kl{is this sentence unique from the last one?} \st{i see. will merge these two sentences} .

In addition, there are two possibilities for estimation and utilization of empowerment: sequential and concurrent. In sequential mode, one firstly estimates empowerment, then utilizes it and/or its byproducts for downstream tasks (\cite{Sharma2020Dynamics-Aware, eysenbach2018diversity}). In concurrent mode, one estimates and utilizes empowerment simultaneously, which is adopted by the current work as well. The concurrent mode is more suitable when the the empowerment objective coincides with the control objective, which happens for instance in stabilization.      

Estimation of mutual information is hard (\cite{mcallester2018formal}). Fortunately, recent advances in deep neural networks (\cite{goodfellow2016deep}) have brought new opportunities for the estimation of mutual information from samples by means of variational low bounds, (VLB), (\cite{poole2019variational, 45903, Tschannen2020On, mohamed2015variational}). However, VLB on empowerment in dynamical control systems (\cite{Sharma2020Dynamics-Aware, achiam2018valor}, [REFS]) have high sample complexity, are often unstable in training \kl{the DADS-Off off policy version of DADS improves on these first two aspects significantly}, and may have a bias [refs] \kl{not sure why there are citations here, VLB is biased by nature?}. Moreover, it was not confirmed previously that VLBs on empowerment do preserve the essential properties of the empowerment function. 

In this work we introduce a new method for empowerment estimation from samples, and utilise the above mentioned property as an "indicator" for the quality of empowerment estimation. Specifically, we propose an alternative path to the estimation of empowerment in dynamical control system, which is based on a particular representation of dynamical control systems by deep neural networks, rather than on VLB. This representation is learnt from samples, (states and actions), and it admits an efficient estimation of empowerment by convex optimization (\cite{cover2012elements}). We propose a unified, (the above mentioned concurrent mode), approach for simultaneous estimation and maximization of empowerment by the off-the-shelf optimisers such as Policy Proximity Optimization, (\cite{1707.06347}) and Stochastic Actor Critic (\cite{1801.01290}). Our method allows us to construct this representation of dynamical systems both from raw states and from images, as demonstrated by numerical simulations.  

Our method is a generic sample-based empowerment estimator. For the sake of clearance of the exposition, and due to the above-mentioned plethora of the possibilities and the applications of empowerment, we put our method on a dedicated testbed, addressing the essential property of the empowerment function, which is the ability to solve the stabilization task with intrinsic reward only.

We believe our experiments convey to the readers in the best way the gist of our method without losing the generality of applicability of our estimator beyond the stabilization task, as we discuss in the future directions.
We demonstrate the advantages of our method by thorough comparisons to the existing state-of-the-art empowerment estimators in different dynamical systems. We found that i) our method has a lower sample complexity, ii) it is more stable in training, iii) it does possess the essential properties of the empowerment function, (while the existing methods do not necessarily do, even though their objective is empowerment maximization as well).

The paper is organised as follows. In Section \ref{sec:Preliminaries} we review the necessary background on reinforcement learning, empowerment, and relevant existing works. In Section \ref{sec:Method} we explain our method. In Section \ref{sec:Experiments}, we provide a) numerical simulations of our method, and) comparison between our method and the existing methods. In Section \ref{sec:Discussion} we summarize the paper, discus the limitations of our method, and propose the continuation which is beyond the scope of the current work.  


==> tex/bck/Introduction.tex.bck.02 <==
\section{Introduction}
Intrinsic motivation allows artificial and biological agents to acquire
useful behaviours without external knowledge (\cite{barto2004intrinsically, NIPS2004_2552, schmidhuber2010formal,  barto2013intrinsic,  oudeyer2016intrinsic}). In the framework of reinforcement learning, (RL), this external domain knowledge is usually provided by an expert through task specific reward, which is optimised by an artificial agent towards desired behaviour (\cite{mnih2013dqn, 1707.06347}). 
% The main disadvantages of this approach are the need to obtain domain knowledge for new environments, and poor generalization to other tasks \kl{I am not sure this is relevant to the benefits of this work} \footnote{The latter can alleviated by meta-learning (\cite{finn2017model}), and goal-conditional policies (\cite{nasiriany2019planning}), which is orthogonal to the main focus of the current **}.  

In contrast, intrinsic reward can arise solely from the interaction between the agent and environment, which eliminate in certain scenarios the need in domain knowledge and reward engineering (\cite{mohamed2015variational, houthooft2017vime, pathak2017curiosity}). Previously, it was shown that maximizing mutual information between agent actuators and its sensors reveals preferable states in environment with regard to the potential to achieve from them a larger number of eventual goals (\cite{klyubin2005all, wissner2013causal}). This potential can be understood by the analogy to the question about where to locate a fire station in a city, such that the firefighters will be able to respond to the largest number of eventual fires on average. Information theoretical quantities allow us to operate with abstract spaces, (such as graph, manifold, language, skill, action, option) through probability distribution, which generalizes the question about positions in Euclidean spaces to points in probability simplex (\cite{cover2012elements}). The subject of this work is intrinsic reward which reflects this potential, and is quantified by the mutual information between actuators and sensors.  

Maximizing this kind of mutual information is known as the empowerment principle (\cite{1554676, salge2014empowerment}). Empowerment is a function of state. It depends only on the properties of agent and environment. Previously, it was shown that an agent maximizing its empowerment converges to unstable equilibrium of environment which was demonstrated on various dynamical control systems (\cite{jung2011empowerment,salge2013approximation,  Karl2019}). In this sense, ascending the gradient of the empowerment function towards unstable equilibrium coincides with the objective of optimal control for stabilization at unstable equilibrium (\cite{strogatz2018nonlinear}) \kl{was it going to be mentioned somewhere around here that empowerment objective is automatically generated for environments, rather than having to hand engineer expert reward functions?}, which is an important task for both engineering (\cite{todorov2006optimal}) and biological\footnote{Broadly speaking, an increase in the rate of information flow in the perception-action loop (\cite{tishby2011information}) could be an impetus for the development of {\it homosapiens}, as hypothesized in (\cite{harari2014}).} systems. It follows from the above mentioned prior works on empowerment that a plausible estimate of the empowerment function should possess this essential property of empowerment. \kl{maybe the last two paragraphs can be made more brief and combined; both describe the empowerment principle (fire station analogy is quite long, and also described as unstable equilibrium)}

    

Empowerment was found useful for a broad spectrum of applications. Among others are unsupervised skill discovery (\cite{Sharma2020Dynamics-Aware, eysenbach2018diversity, DBLP:conf/iclr/GregorRW17, Karl2019, EDL2020}), human-agent coordination (\cite{Salge2017EmpowermentAR,guckelsberger2016intrinsically}),  assistance (\cite{AvE2020}), and stabilization (\cite{tiomkin2017control}). In general, in these applications, the agent maximizes mutual information between its actuators, which generate either action as in (\cite{Karl2019,DBLP:conf/iclr/GregorRW17}), or action sequence as in (\cite{tiomkin2017unified, salge2014empowerment}), or options as in (\cite{DBLP:conf/iclr/GregorRW17}), or skills as in (\cite{Sharma2020Dynamics-Aware, eysenbach2018diversity}) and its sensors. 

In addition, there are two possibilities for estimation and utilization of empowerment: sequential and concurrent. In sequential mode, one firstly estimates empowerment, then utilizes it and/or its byproducts for downstream tasks (\cite{Sharma2020Dynamics-Aware, eysenbach2018diversity}). In concurrent mode, one estimates and utilizes empowerment simultaneously, which is adopted by the current work as well. The concurrent mode is more suitable when the the empowerment objective coincides with the control objective, which happens for instance in stabilization.      

Estimation of mutual information is hard (\cite{mcallester2018formal}). Fortunately, recent advances in deep neural networks (\cite{goodfellow2016deep}) have brought new opportunities for the estimation of mutual information from samples by means of variational low bounds, (VLB), (\cite{poole2019variational, 45903, Tschannen2020On, mohamed2015variational}). However, VLB on empowerment in dynamical control systems (\cite{Sharma2020Dynamics-Aware, achiam2018valor}) have high sample complexity, are often unstable in training, and may have a bias. Moreover, it was not confirmed previously that VLBs on empowerment do preserve the essential properties of the empowerment function. 

In this work we introduce a new method for empowerment estimation from samples, and utilise the above mentioned property as an "indicator" for the quality of empowerment estimation. Specifically, we propose an alternative path to the estimation of empowerment in dynamical control system, which is based on a particular representation of dynamical control systems by deep neural networks, rather than on VLB. This representation is learnt from samples, (states and actions), and it admits an efficient estimation of empowerment by convex optimization (\cite{cover2012elements}). We propose a unified, (the above mentioned concurrent mode), approach for simultaneous estimation and maximization of empowerment by the off-the-shelf optimisers such as Policy Proximity Optimization, (\cite{1707.06347}) and Stochastic Actor Critic (\cite{1801.01290}). Our method allows us to construct this representation of dynamical systems both from raw states and from images, as demonstrated by numerical simulations.  

Our method is a generic sample-based empowerment estimator. For the sake of clearance of the exposition, and due to the above-mentioned plethora of the possibilities and the applications of empowerment, we put our method on a dedicated testbed, addressing the essential property of the empowerment function, which is the ability to solve the stabilization task with intrinsic reward only.

We believe our experiments convey to the readers in the best way the gist of our method without losing the generality of applicability of our estimator beyond the stabilization task, as we discuss in the future directions. We demonstrate the advantages of our method by thorough comparisons to the existing state-of-the-art empowerment estimators in different dynamical systems. We found that i) our method has a lower sample complexity, ii) it is more stable in training, iii) it does possess the essential properties of the empowerment function, while the existing methods do not.

The paper is organised as follows. In Section \ref{sec:Preliminaries} we review the necessary background on reinforcement learning, empowerment, and relevant existing works. In Section \ref{sec:Method} we explain our method. In Section \ref{sec:Experiments}, we provide a) numerical simulations of our method, and) comparison between our method and the existing methods. In Section \ref{sec:Discussion} we summarize the paper, discus the limitations of our method, and propose the continuation which is beyond the scope of the current work.  
